Nova-LSM: A Distributed, Component-based LSM-tree Key-value Store

The cloud infrastructure motivates disaggregation of monolithic data stores into components that are assembled together based on an application's workload. This study investigates disaggregation of an LSM-tree key-value store into components that communicate using RDMA. These components separate storage from processing, enabling processing components to share storage bandwidth and space. The processing components scatter blocks of a file (SSTable) across an arbitrary number of storage components and balance load across them using power-of-d. They construct ranges dynamically at runtime to parallelize compaction and enhance performance. Each component has configuration knobs that control its scalability. The resulting component-based system, Nova-LSM, is elastic. It outperforms its monolithic counterparts, both LevelDB and RocksDB, by several orders of magnitude with workloads that exhibit a skewed pattern of access to data.

==> conclusion.tex <==
\section{Conclusion and Future Work}\label{sec:conclusion}
Nova-LSM is a component-based implementation of LSM-tree that separates storage from processing using RDMA.  
It provides significant performance benefits when compared with a traditional LSM-tree implementation.
It provides the highest benefits (several orders of magnitude) with workloads that exhibit a skewed pattern of access to data.  

We are extending Nova-LSM in several exciting directions.  
As highlighted by the horizontal scalability discussions of Section~\ref{sec:eval:horizontal-scale}, the number of LTCs and StoCs has a profound impact on both the performance and scalability of a deployment.  
At the same time, Nova-LSM is highly elastic.  
We are exploring the feasibility of an online planner that monitors a deployment and adjusts its number of LTCs and StoCs dynamically to realize the highest price/performance for a workload.


